Learning Interpretable Temporal Properties from Positive Examples Only

We consider the problem of explaining the temporal behavior of black-box systems using human-interpretable models. To this end, based on recent research trends, we rely on the fundamental yet interpretable models of deterministic finite automata (DFAs) and linear temporal logic (LTL) formulas. In contrast to most existing works for learning DFAs and LTL formulas, we rely on only positive examples. Our motivation is that negative examples are generally difficult to observe, in particular, from black-box systems. To learn meaningful models from positive examples only, we design algorithms that rely on conciseness and language minimality of models as regularizers. To this end, our algorithms adopt two approaches: a symbolic and a counterexample-guided one. While the symbolic approach exploits an efficient encoding of language minimality as a constraint satisfaction problem, the counterexample-guided one relies on generating suitable negative examples to prune the search. Both the approaches provide us with effective algorithms with theoretical guarantees on the learned models. To assess the effectiveness of our algorithms, we evaluate all of them on synthetic data.

==> resources/Makefile <==


all: plots/UAV.pdf plots/LTLf.pdf plots/LTLf2.pdf

plots/UAV.pdf: plot_traces.py $(shell ls -d stats/uav/**)
	@mkdir -p $(dir $@)
	./$<

plots/LTLf.pdf plots/LTLf2.pdf: plot_traces.py $(subst :,\:,$(shell ls -d stats/ltlf/**))
	@mkdir -p $(dir $@)
	./$<

